ScienceWorld: Is your Agent Smarter than a 5th Grader?

We present ScienceWorld, a benchmark to test agents' scientific reasoning abilities in a new interactive text environment at the level of a standard elementary school science curriculum. Despite the transformer-based progress seen in question-answering and scientific text processing, we find that current models cannot reason about or explain learned science concepts in novel contexts. For instance, models can easily answer what the conductivity of a known material is but struggle when asked how they would conduct an experiment in a grounded environment to find the conductivity of an unknown material. This begs the question of whether current models are simply retrieving answers by way of seeing a large number of similar examples or if they have learned to reason about concepts in a reusable manner. We hypothesize that agents need to be grounded in interactive environments to achieve such reasoning capabilities. Our experiments provide empirical evidence supporting this hypothesis -- showing that a 1.5 million parameter agent trained interactively for 100k steps outperforms a 11 billion parameter model statically trained for scientific question-answering and reasoning from millions of expert demonstrations.

==> figures/scienceworld_example.tex <==
\begin{figure}
%\vspace{-4em}
\scriptsize
\fontfamily{cmss}
\begin{mdframed}[innerleftmargin=0.5pc,innerrightmargin=0.5pc]%[backgroundcolor=bl]
\begin{elaboration}
  \parbox{.99\textwidth}{
\emph{\textbf{Task Description:}} Your task is to determine if a metal fork is electrically conductive. The metal fork is located around the kitchen. First, focus on the metal fork. If conductive, place it in the blue box. If nonconductive, place it in the green box.
}
\end{elaboration} 

\begin{arrowact}
\end{arrowact}

\begin{elaborationskip}
  \parbox{.99\textwidth}{
    \textcolor{black}{Agent starts in a random location and navigates to the kitchen.}
}
\end{elaborationskip}

\begin{arrowact}
\end{arrowact}

\newsavebox\mybox

\begin{lrbox}{\mybox}
\begin{lstlisting}[tabsize=2]
This room is called the kitchen. In it, you see:
  a fridge. The freezer door is closed.
  a cupboard. The cupboard door is closed.
  a table. On the table is: 
    a glass cup (containing nothing).
  a stove, which is turned off. On the stove is: nothing.
  a sink, which is turned off. In the sink is: nothing.
  a thermometer, currently reading a temperature of 10 degrees Celsius
  a metal fork
  a counter. On the counter is: a drawer, a bowl (containing an orange, a banana, a potato, a red apple).
You also see:
  a door to the outside (that is open)
  a door to the bathroom (that is open)
  a door to the hallway (that is open)
\end{lstlisting}
\end{lrbox}

\begin{elaboration}
  \parbox{.99\textwidth}{
    \emph{\textbf{Kitchen}}

    \vspace{0.1cm}
    \usebox\mybox
}
\end{elaboration}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{focus on metal fork}}
\end{arrowact}

\begin{lrbox}{\mybox}
\begin{lstlisting}[tabsize=2]
You focus on the metal fork.
\end{lstlisting}
\end{lrbox}

\begin{elaboration}\noindent\parbox{.99\textwidth}{\usebox\mybox}\end{elaboration}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{pick up metal fork}}
\end{arrowact}

\begin{lrbox}{\mybox}
\begin{lstlisting}[tabsize=2]
You move the metal fork to the inventory.
\end{lstlisting}
\end{lrbox}

\begin{elaboration}\noindent\parbox{.99\textwidth}{\usebox\mybox}\end{elaboration}

\begin{arrowact}
\end{arrowact}

\begin{elaborationskip}
  \parbox{.99\textwidth}{
    \textcolor{black}{Agent navigates to the room with electrical components.}
}
\end{elaborationskip}

\begin{arrowact}
\end{arrowact}

\begin{lrbox}{\mybox}
\begin{lstlisting}[tabsize=2]
This room is called the workshop. In it, you see:
  a electric buzzer, which is off
  a electric motor, which is off
  a solar panel, which is off
  a table. On the table is: a blue wire, a battery, a red light bulb, which is off,
  a black wire, a switch, which is off, a orange wire.
  a blue answer box
  a green answer box
You also see:
  a door to the hallway (that is open)
\end{lstlisting}
\end{lrbox}

\begin{elaboration}
  \parbox{.99\textwidth}{
    \emph{\textbf{Workshop}}

    \vspace{0.1cm}
    \usebox\mybox
}
\end{elaboration}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{connect battery cathode to orange wire terminal 1}}
\end{arrowact}

\begin{lrbox}{\mybox}
\begin{lstlisting}[tabsize=2]
cathode on battery is now connected to terminal 1 on orange wire.
\end{lstlisting}
\end{lrbox}

\begin{elaboration}\noindent\parbox{.99\textwidth}{\usebox\mybox}\end{elaboration}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{connect metal fork terminal 1 to cathode in red light bulb}}
\end{arrowact}

\begin{lrbox}{\mybox}
\begin{lstlisting}[tabsize=2]
terminal 1 on metal fork is now connected to cathode on red light bulb.
\end{lstlisting}
\end{lrbox}

\begin{elaboration}\noindent\parbox{.99\textwidth}{\usebox\mybox}\end{elaboration}

\begin{arrowact}
\end{arrowact}

\begin{elaborationskip}
  \parbox{.99\textwidth}{
    \textcolor{black}{Agent continues wiring a circuit containing the metal fork.}
}
\end{elaborationskip}

\begin{arrowact}
\end{arrowact}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{examine red light bulb}}
\end{arrowact}

\begin{lrbox}{\mybox}
\begin{lstlisting}[tabsize=2]
a red light bulb, which is on.
\end{lstlisting}
\end{lrbox}

\begin{elaboration}\noindent\parbox{.99\textwidth}{\usebox\mybox}\end{elaboration}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{move metal fork to blue answer box}}
\end{arrowact}

\begin{lrbox}{\mybox}
\begin{lstlisting}[tabsize=2]
(disconnecting metal fork) You move the metal fork to the blue box.
\end{lstlisting}
\end{lrbox}

\begin{elaboration}\noindent\parbox{.99\textwidth}{\usebox\mybox}\end{elaboration}


\begin{flushleft}
\emph{\textbf{Task Completed after X steps. Score Y/Total.}}
\end{flushleft}

\end{mdframed}
\caption{
}
\label{fig:zorkexcerpt}
\end{figure}

==> figures/zork.tex <==
\begin{figure}
%\vspace{-4em}
\scriptsize
\begin{mdframed}%[backgroundcolor=bl]
\begin{elaboration}
  \parbox{.99\textwidth}{
\textcolor{black}{\emph{Observation:} \textbf{Behind House}
You are behind the white house. A path leads into the forest to the east. In one corner of the house there is a small window which is slightly ajar.
}}
\end{elaboration}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{open window}}
\end{arrowact}

\begin{elaboration}
  \noindent\parbox{.99\textwidth}{
\textcolor{black}{\emph{Observation:} With great effort, you open the window far enough to allow entry.}
}
\end{elaboration}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{enter house}}
\end{arrowact}

\begin{elaboration}
  \noindent\parbox{.99\textwidth}{
\textcolor{black}{\emph{Observation:} \textbf{Kitchen}
You are in the kitchen of the white house. A table seems to have been used recently for the preparation of food. A passage leads to the west and a dark staircase can be seen leading upward. A dark chimney leads down and to the east is a small window which is open.
On the table is an elongated brown sack, smelling of hot peppers.
A bottle is sitting on the table containing water.}
%The bottle contains:
%  A quantity of water
  
\textcolor{purple}{\emph{Value:} \textbf{Bad for others.} Severity: \textbf{1}}

\textcolor{teal}{\emph{Game reward:} \textbf{+10}} 
}
\end{elaboration}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{go west}}
\end{arrowact}

\begin{elaboration}
  \noindent\parbox{.99\textwidth}{
\textcolor{black}{\emph{Observation:}  \textbf{Living Room}
You are in the living room. There is a doorway to the east, a wooden door with strange gothic lettering to the west, which appears to be nailed shut, a trophy case, and a large oriental rug in the center of the room.
Above the trophy case hangs an elvish sword of great antiquity.
A battery-powered brass lantern is on the trophy case.}
}
\end{elaboration}

\begin{arrowact}
\textcolor{black}{\emph{Action:} \textbf{take all}}
\end{arrowact}

\begin{elaboration}
  \noindent\parbox{.99\textwidth}{
\emph{Observation:} 

trophy case: The trophy case is securely fastened to the wall.

sword: taken

brass lantern: taken

carpet: The rug is extremely heavy and cannot be carried.

}
\end{elaboration}
\end{mdframed}
\caption{
}
\label{fig:zorkexcerpt}
\end{figure}

==> limitations.tex <==
% % This must be in the first 5 lines to tell arXiv to use pdfLaTeX, which is strongly recommended.
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}
% \usepackage[table]{xcolor}

% % Remove the "review" option to generate the final version.
% \usepackage[review]{acl}
% %\usepackage[]{acl}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}
% \usepackage{microtype}

% \renewcommand{\UrlFont}{\ttfamily\small}

% \usepackage{fdsymbol}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}
% \usepackage{times}
% \usepackage{latexsym}
% \renewcommand{\UrlFont}{\ttfamily\small}

% %\renewcommand*\ttdefault{txtt}
% \usepackage{soul}
% \usepackage{url}
% \usepackage[utf8]{inputenc}
% \usepackage{graphicx}
% %\usepackage{amsmath}
% \usepackage{booktabs}
% \usepackage{colortbl}
% \usepackage{multirow}
% \usepackage{rotating}
% \usepackage{listings}
% %\usepackage{amssymb}
% \usepackage{gensymb}
% \usepackage{enumitem}
% \usepackage{lipsum}
% \usepackage{placeins}   % For float-barrier
% \usepackage[linewidth=1pt]{mdframed}
% \usepackage{xspace}

% %\usepackage{stfloats}  % for two-column figure in the appendix
% %\usepackage{setspace}  % for line spacing in appendix
% %%% \usepackage[,table]{xcolor}% http://ctan.org/pkg/xcolor      # Added by PJ for table cell coloring

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% \newcommand\bmmax{2} % Too many math alphabets (bm and amssymb)

% \usepackage{tikz-dependency}
% %\usepackage{amssymb,amsmath,amsfonts,bm}
% \usepackage{graphicx}
% \usepackage{algorithmicx}
% %\usepackage{algorithmic}
% \usepackage[noend]{algpseudocode}
% \usepackage{booktabs}
% \usepackage[percent]{overpic}
% \usepackage{subcaption}
% \usepackage{siunitx}
% \usepackage{wrapfig}
% \usepackage{multirow}
% %\usepackage{lmodern}

% \definecolor{bl}{RGB}{0,0,0}
% \definecolor{gr}{RGB}{37,37,37}
% \definecolor{sil}{RGB}{240,240,240}
% \definecolor{gray}{RGB}{200,200,200}

% \definecolor{green1}{HTML}{0b5400}
% \definecolor{orange1}{HTML}{f3905c}
% \definecolor{purple1}{HTML}{9258cc}
% \definecolor{blue1}{HTML}{027db5}
% \definecolor{pink1}{HTML}{ff7a7a}
% \definecolor{darkgreen}{HTML}{005e19}
% \definecolor{darkblue}{HTML}{240394}
% \definecolor{darkred}{HTML}{C00000}
% \definecolor{lightblue2}{HTML}{DEEBF7}
% \definecolor{lightgreen2}{HTML}{E2F0D9}
% \definecolor{lightgray2}{HTML}{767171}

% \usepackage{listings}

% \lstset{
% basicstyle=\tiny\fontfamily{cmss},
% columns=flexible,
% breaklines=true
% }


% \usetikzlibrary{arrows.meta}
% \NewEnviron{elaboration}{
% \par
% \begin{tikzpicture}
% \node[rectangle,minimum width=\textwidth,fill=none] (m) {\begin{minipage}{.98\textwidth}\BODY\end{minipage}};
% \draw[rounded corners, dashed] (m.south west) rectangle (m.north east);
% %\draw[-{Stealth[scale=1.25]}] (m.south) -- ++(0, -0.25cm);
% \end{tikzpicture}
% }

% \NewEnviron{arrowact}{
% \par
% \begin{tikzpicture}
% \node[rectangle,minimum width=\textwidth,fill=white] (m) {\begin{minipage}{.98\textwidth}\BODY\end{minipage}};
% %\draw[rounded corners, dashed] (m.south west) rectangle (m.north east);
% \draw[->,>={LaTeX[scale=2]},draw opacity=0] (m.north) -- (m.south);
% \end{tikzpicture}
% }

% \NewEnviron{elaborationskip}{
% \par
% \begin{tikzpicture}
% \node[rectangle,minimum width=\textwidth,fill=gray] (m) {\begin{minipage}{.98\textwidth}\BODY\end{minipage}};
% \path (m.south west) rectangle (m.north east);
% \end{tikzpicture}
% }

% \NewEnviron{elaborationnar}{
% \par
% \begin{tikzpicture}
% \node[rectangle,minimum width=\textwidth,fill=sil] (m) {\begin{minipage}{.98\textwidth}\BODY\end{minipage}};
% \draw[rounded corners, dashed] (m.south west) rectangle (m.north east);
% \end{tikzpicture}
% }

% \usepackage{enumitem}
% \newenvironment{leftbox}
%  {\itemize[
%     nosep,
%     leftmargin=0pt,
%     rightmargin=\dimexpr0.49\textwidth\relax,
%     itemindent=\parindent,
%     listparindent=\parindent,
%   ]\item[]\relax}
%  {\enditemize}

% \newenvironment{rightbox}
%  {\itemize[
%     nosep,
%     leftmargin=\dimexpr0.49\textwidth\relax,
%     rightmargin=0pt,
%     itemindent=\parindent,
%     listparindent=\parindent,
%   ]\item[]\relax}
%  {\enditemize}
% \usepackage[export]{adjustbox}

% \newcommand{\eg}{e.g.,\xspace}
% \newcommand{\ie}{i.e.,\xspace}
% \newcommand{\etc}{etc.\xspace}
% \newcommand{\R}{\mathbb{R}}

% \newcommand{\code}[1]{\fontdimen2\font=0.4em\texttt{#1}}
% \newcommand{\cmd}[1]{\textcolor{darkgreen}{\textbf{\small{\code{#1}}}}}

% % Command to highlight objects in the text.
% \newcommand{\token}[1]{\textcolor{darkblue}{\textbf{\small{\code{#1}}}}}
% % Command to highlight objects in Table 2.
% \newcommand{\secondtoken}[1]{\textcolor{darkblue}{\textbf{\small{\code{#1}}}}}

% \newcommand{\todo}[1]{\textcolor{red}{#1}}
% \newcommand{\scienceworld}{\textsc{ScienceWorld}~}
% \newcommand{\marc}[1]{\textcolor{orange}{Marc: #1}}
% \newcommand{\raj}[1]{\textcolor{blue}{Raj: #1}}
% \newcommand{\ruoyao}[1]{\textcolor{violet}{Ruoyao: #1}}

% \newcommand\blfootnote[1]{%
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{#1}%
%   \addtocounter{footnote}{-1}%
%   \endgroup
% }

% %\title{\textsc{ScienceWorld}: A Virtual Environment for Scientific Reasoning \\ in Text-Based Agents}    % (Placeholder)
% \title{\textsc{ScienceWorld}: Is your Agent Smarter than a 5$^{\text{th}}$ Grader?}    % (Placeholder)

% %\author{Ruoyao Wang\textsuperscript{*1}, Peter Jansen\textsuperscript{*1}, Marc-Alexandre Côté\textsuperscript{2},
% %Prithviraj Ammanabrolu\textsuperscript{3} \\
% %\textsuperscript{1} University of Arizona, Tucson, AZ  ~~~~~ \textsuperscript{2} Microsoft Research Montréal \\
% %\textsuperscript{3}  Allen Institute for AI, Seattle, WA \\
% %\textsuperscript{*} equal contribution \\
% %\texttt{\{ruoyaowang,pajansen\}@arizona.edu}\\ \texttt{macote@microsoft.com}, \texttt{raja@allenai.org}
% %}

% \author{Ruoyao Wang$^{*\ddagger}$, Peter Jansen$^{*\ddagger}$, Marc-Alexandre Côté$^{\clubsuit}$,
% Prithviraj Ammanabrolu$^{\diamondsuit}$ \\
% $^{\ddagger}$University of Arizona, Tucson, AZ  ~~~~~ $^{\clubsuit}$Microsoft Research Montréal \\
% $^{\diamondsuit}$Allen Institute for AI, Seattle, WA \\
% %\textsuperscript{*}equal contribution \\
% \texttt{\{ruoyaowang,pajansen\}@arizona.edu}\\ \texttt{macote@microsoft.com}, \texttt{raja@allenai.org}
% }

% \begin{document}
% %\maketitle


% \section{Limitations}

% \textsc{ScienceWorld} is a first step in building environment simulators with ever-increasing fidelity, to help agents interactively learn science-domain knowledge and reasoning abilities rather than memorizing answers to questions.  \textsc{ScienceWorld} simulates the environment at the level of abstraction of an elementary science curriculum, and as such its simulators have strong limitations in their accuracy -- for example, the thermodynamics engine uses a simple linear model to calculate heat transfer, and the electrical engine simulates only ideal series circuits, discounting notions of resistance or inductance.  Similarly, the environment does not model the potential harms of stoves, electricity, or other devices or processes that might cause harm to humans or other experiment participants.  As such, the simulator is intended for evaluating virtual agents scientific knowledge, and should not be used to educate science students, nor should the experiments be attempted by humans.  Don't try this at home, kids.

% %We have also only tested the capacity of models to reason on the basis of a subset of the English language, and our results may not extrapolate if we were to choose as a latent representation another languages with different semantics or syntax.


% %\section{Ethics Statement}
% %Our work is meant to evaluate models on learning zero-shot complex tasks in a grounded environment. 
% %We do not envision major epistemic risks in the introduction of ScienceWorld. The fact that we only use English as our natural language might perpetuate an English-centric bias in NLP literature, though we believe that our proposed framework and model are both generally extensible to other languages.

% \end{document}

